Hey Alexa what did I just type? Decoding smartphone sounds with a voice assistant

Voice assistants are now ubiquitous and listen in on our everyday lives. Ever since they became commercially available, privacy advocates worried that the data they collect can be abused: might private conversations be extracted by third parties? In this paper we show that privacy threats go beyond spoken conversations and include sensitive data typed on nearby smartphones. Using two different smartphones and a tablet we demonstrate that the attacker can extract PIN codes and text messages from recordings collected by a voice assistant located up to half a meter away. This shows that remote keyboard-inference attacks are not limited to physical keyboards but extend to virtual keyboards too. As our homes become full of always-on microphones, we need to work through the implications.

==> TDoA-hyperbolae.5.tex <==
%\usepackage[utf8]{inputenc}
%\usepackage{pgf,tikz,pgfplots}
%\pgfplotsset{compat=1.15}
%\usepackage{mathrsfs}
%\usetikzlibrary{arrows}
%\pagestyle{empty}
\definecolor{ududff}{rgb}{0.30196078431372547,0.30196078431372547,1.}
\definecolor{uuuuuu}{rgb}{0.26666666666666666,0.26666666666666666,0.26666666666666666}
\definecolor{zzttqq}{rgb}{0.6,0.2,0.}
\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1.}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm,scale=0.3]
%\begin{axis}[
%x=1.0cm,y=1.0cm,
%axis lines=none,
%ymajorgrids=false,
%xmajorgrids=false,
%xmin=-9.055097946802741,
%xmax=9.08601671751565,
%ymin=-18.520828089899275,
%ymax=5.713066386036061,
%xtick={},
%ytick={},]
\node[inner sep=0pt] (image) at (0,-11.75){\includegraphics[scale=0.075]{figs/screenshot-flounder-landscape-word.png}};
\clip(-9.055097946802741,-18.520828089899275) rectangle (9.08601671751565,5.713066386036061);
\fill[line width=.5pt,color=zzttqq,fill=zzttqq,fill opacity=0.10000000149011612] (4.63,0.) -- (2.315,4.00969761952195) -- (-2.315,4.009697619521951) -- (-4.63,0.) -- (-2.315,-4.009697619521951) -- (2.315,-4.009697619521953) -- cycle;
\draw [line width=.5pt,color=zzttqq] (4.63,0.)-- (2.315,4.00969761952195);
\draw [line width=.5pt,color=zzttqq] (2.315,4.00969761952195)-- (-2.315,4.009697619521951);
\draw [line width=.5pt,color=zzttqq] (-2.315,4.009697619521951)-- (-4.63,0.);
\draw [line width=.5pt,color=zzttqq] (-4.63,0.)-- (-2.315,-4.009697619521951);
\draw [line width=.5pt,color=zzttqq] (-2.315,-4.009697619521951)-- (2.315,-4.009697619521953);
\draw [line width=.5pt,color=zzttqq] (2.315,-4.009697619521953)-- (4.63,0.);
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({1.9495781250000004*(1+(\x)^2)/(1-(\x)^2)},{1.2483469607931446*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({1.9495781250000004*(-1-(\x)^2)/(1-(\x)^2)},{1.2483469607931446*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({1.5951093750000003*(1+(\x)^2)/(1-(\x)^2)},{1.6777517938560251*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({1.5951093750000003*(-1-(\x)^2)/(1-(\x)^2)},{1.6777517938560251*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({1.2406406250000006*(1+(\x)^2)/(1-(\x)^2)},{1.9544911971148935*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({1.2406406250000006*(-1-(\x)^2)/(1-(\x)^2)},{1.9544911971148935*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({0.8861718749999999*(1+(\x)^2)/(1-(\x)^2)},{2.1386735159811048*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({0.8861718749999999*(-1-(\x)^2)/(1-(\x)^2)},{2.1386735159811048*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({0.531703125*(1+(\x)^2)/(1-(\x)^2)},{2.2531126884524073*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({0.531703125*(-1-(\x)^2)/(1-(\x)^2)},{2.2531126884524073*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521951)},xshift=0.cm,yshift=-4.009697619521951cm,line width=.5pt] plot ({0.17723437499999994*(1+(\x)^2)/(1-(\x)^2)},{2.308205574969085*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521951)},xshift=0.cm,yshift=-4.009697619521951cm,line width=.5pt] plot ({0.17723437499999994*(-1-(\x)^2)/(1-(\x)^2)},{2.308205574969085*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({2.304046875000054*(1+(\x)^2)/(1-(\x)^2)},{0.22492887276366766*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.5pt] plot ({2.304046875000054*(-1-(\x)^2)/(1-(\x)^2)},{0.22492887276366766*(-2)*(\x)/(1-(\x)^2)});
\begin{scriptsize}
\draw [fill=xdxdff] (4.63,0.) circle (2.5pt);
\draw [fill=xdxdff] (2.315,4.00969761952195) circle (2.5pt);
\draw [fill=uuuuuu] (-2.315,4.009697619521951) circle (2.5pt);
\draw [fill=uuuuuu] (-4.63,0.) circle (2.5pt);
\draw [fill=uuuuuu] (-2.315,-4.009697619521951) circle (2.5pt);
\draw [fill=uuuuuu] (2.315,-4.009697619521953) circle (2.5pt);
\draw [fill=ududff] (-9.04,-18.5) circle (2.5pt);
\draw [fill=ududff] (9.04,-18.5) circle (2.5pt);
\end{scriptsize}
%\end{axis}
\end{tikzpicture}


==> TDoA-hyperbolae.tex <==
%\usepackage[utf8]{inputenc}
%\usepackage{pgf,tikz,pgfplots}
%\pgfplotsset{compat=1.15}
%\usepackage{mathrsfs}
%\usetikzlibrary{arrows}
\pagestyle{empty}
\definecolor{ududff}{rgb}{0.30196078431372547,0.30196078431372547,1.}
\definecolor{uuuuuu}{rgb}{0.26666666666666666,0.26666666666666666,0.26666666666666666}
\definecolor{zzttqq}{rgb}{0.6,0.2,0.}
\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1.}
\begin{tikzpicture}[scale=0.3,line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\begin{axis}[
x=1.0cm,y=1.0cm,
axis lines=middle,
ymajorgrids=true,
xmajorgrids=true,
xmin=-9.197774673337571,
xmax=9.829621505049058,
ymin=-15.47727693152653,
ymax=4.22703499484575,
xtick={-8.0,-6.0,...,8.0},
ytick={-18.0,-16.0,...,4.0},]
\node[inner sep=0pt] (image) at (0,-11.75)
{\includegraphics[scale=0.0751]{figs/screenshot-flounder-landscape-word.png}};
\clip(-9.197774673337571,-18.47727693152653) rectangle (9.829621505049058,4.22703499484575);
\fill[line width=2.pt,color=zzttqq,fill=zzttqq,fill opacity=0.10000000149011612] (4.63,0.) -- (2.315,4.00969761952195) -- (-2.315,4.009697619521951) -- (-4.63,0.) -- (-2.315,-4.009697619521951) -- (2.315,-4.009697619521953) -- cycle;
\draw [line width=.7pt,color=zzttqq] (4.63,0.)-- (2.315,4.00969761952195);
\draw [line width=.7pt,color=zzttqq] (2.315,4.00969761952195)-- (-2.315,4.009697619521951);
\draw [line width=.7pt,color=zzttqq] (-2.315,4.009697619521951)-- (-4.63,0.);
\draw [line width=.7pt,color=zzttqq] (-4.63,0.)-- (-2.315,-4.009697619521951);
\draw [line width=.7pt,color=zzttqq] (-2.315,-4.009697619521951)-- (2.315,-4.009697619521953);
\draw [line width=.7pt,color=zzttqq] (2.315,-4.009697619521953)-- (4.63,0.);
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({2.1268125000000015*(1+(\x)^2)/(1-(\x)^2)},{0.9142721639882458*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({2.1268125000000015*(-1-(\x)^2)/(1-(\x)^2)},{0.9142721639882458*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({1.7723437499999999*(1+(\x)^2)/(1-(\x)^2)},{1.489302733441369*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({1.7723437499999999*(-1-(\x)^2)/(1-(\x)^2)},{1.489302733441369*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({1.417875000000001*(1+(\x)^2)/(1-(\x)^2)},{1.8299878372205107*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({1.417875000000001*(-1-(\x)^2)/(1-(\x)^2)},{1.8299878372205107*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({1.06340625*(1+(\x)^2)/(1-(\x)^2)},{2.056305460640743*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({1.06340625*(-1-(\x)^2)/(1-(\x)^2)},{2.056305460640743*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({0.7089375000000007*(1+(\x)^2)/(1-(\x)^2)},{2.2037768991197257*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({0.7089375000000007*(-1-(\x)^2)/(1-(\x)^2)},{2.2037768991197257*(-2)*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({0.3544687500000003*(1+(\x)^2)/(1-(\x)^2)},{2.2877012272745407*2*(\x)/(1-(\x)^2)});
\draw [samples=50,domain=-0.99:0.99,rotate around={0.:(0.,-4.009697619521952)},xshift=0.cm,yshift=-4.009697619521952cm,line width=.7pt] plot ({0.3544687500000003*(-1-(\x)^2)/(1-(\x)^2)},{2.2877012272745407*(-2)*(\x)/(1-(\x)^2)});
\draw [line width=.7pt] (0.,-18.47727693152653) -- (0.,4.22703499484575);
\draw [line width=.7pt] (0.,-18.47727693152653) -- (0.,4.22703499484575);
\begin{scriptsize}
\draw [fill=xdxdff] (4.63,0.) circle (2.5pt);
\draw [fill=xdxdff] (2.315,4.00969761952195) circle (2.5pt);
\draw [fill=uuuuuu] (-2.315,4.009697619521951) circle (2.5pt);
\draw [fill=uuuuuu] (-4.63,0.) circle (2.5pt);
\draw [fill=uuuuuu] (-2.315,-4.009697619521951) circle (2.5pt);
\draw [fill=uuuuuu] (2.315,-4.009697619521953) circle (2.5pt);
\draw [fill=uuuuuu] (0.,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (0.3544687499999979,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (0.708937499999998,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (1.0634062499999977,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (1.4178749999999978,-4.009697619521953) circle (2.0pt);
\draw [fill=uuuuuu] (1.7723437499999979,-4.009697619521953) circle (2.0pt);
\draw [fill=uuuuuu] (2.1268124999999976,-4.009697619521953) circle (2.0pt);
\draw [fill=uuuuuu] (-0.35446875000000233,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (-0.7089375000000022,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (-1.063406250000002,-4.009697619521952) circle (2.0pt);
\draw [fill=uuuuuu] (-1.4178750000000022,-4.009697619521951) circle (2.0pt);
\draw [fill=uuuuuu] (-1.7723437500000023,-4.009697619521951) circle (2.0pt);
\draw [fill=uuuuuu] (-2.126812500000002,-4.009697619521951) circle (2.0pt);
\draw [fill=ududff] (-9.04,-18.5) circle (2.5pt);
\draw [fill=ududff] (9.04,-18.5) circle (2.5pt);
\end{scriptsize}
\end{axis}
\end{tikzpicture}


==> abstract-clean.tex <==
\newpage
{\Huge \bf Abstract}
\vspace{24pt} 


Write a summary of the whole thing. Make 
sure it fits in one page. 


\newpage
\vspace*{\fill}


==> abstract.tex <==
\ifeven\value{page}\hbox{}\newpage\fi
{\large \bf Detecting taps on a keyboard using a smart speaker microphone}
\vspace{24pt} 

\textbf{Abstract}

The growing popularity of smart speakers like the Amazon Echo raises privacy concerns of microphones
in a home. They overhear conversations and other noises which they send to the cloud service. 
It has been shown that computer keyboards emit a lot of noise on each keystroke, and this can be
used to reconstruct the text that was entered. In this dissertation, I perform a similar attack on
virtual keyboards. These are harder to attack as their tapping makes a
shorter and fainter sound that easily gets lost in noise. 
There have been successful attacks that make use of the internal microphone on the device. 
In this work, we use an external microphone array. 
We can detect \SIrange{75}{80}{\percent} of taps on a touchscreen about \SI{20}{\centi\metre} away
from the array, and can identify around \SI{40}{\percent} of both numeric digits and English
letters on the first guess. When detection works well, we can guess about \SI{40}{\percent} of
English dictionary words in 10 guesses. 

\newpage
\vspace*{\fill}


==> acknowledgements.tex <==
\newpage
{\Huge \bf Acknowledgements}

\vspace{24pt} 

Suppressed for anonymous review.

%I would like to thank Ilia Shumailov for suggesting the project and supervising me, and Ross Anderson and John Fawcett for giving me feedback on my work. I would like to thank my father Akos Zarandy for sharing his slides on convolutional neural networks with me, and my mother and brother for providing data for evaluation of my project. 

\newpage
\vspace*{\fill}


==> declaration.tex <==
\newpage
{\Huge \bf Declaration}

\vspace{24pt} 

I \authorname of \authorcollege, being a candidate for Computer Science Tripos, Part III, hereby declare that this report and the
work described in it are my own work, unaided except as may be
specified below, and that the report does not contain material that
has already been used to any substantial extent for a comparable
purpose.

\vspace{24pt}
Total word count: \input{count.txt}

\vspace{60pt}
\textbf{Signed}: 
Almos Zarandy

\vspace{12pt}
\textbf{Date}:
03/06/2020

\vfill

This dissertation is copyright \copyright 2020 \authorname. 
\\
All trademarks used in this dissertation are hereby acknowledged.



\newpage
\vspace*{\fill}

